Medical Imaging Classification with Cold-Atom Reservoir Computing using Auto-Encoders and Surrogate-Driven Training

We introduce a hybrid quantum-classical pipeline, based on neutral-atom reservoir computing, for medical image classification, focusing on the binary classification task of polyp detection. To deal effectively with the high dimensionality, we integrate a guided auto-encoder. This pipeline learns compact and discriminative representations of image data that are also well-suited for quantum reservoir computing. A key challenge in such systems is the non-differentiable nature of quantum measurements, which creates a 'gradient barrier' for standard training. We overcome this barrier by incorporating a differentiable surrogate model that emulates the quantum layer, enabling end-to-end backpropagation through the entire system. This guided training process is jointly optimized for classification accuracy and for faithful image recovery from the auto-encoder. The learned latent representations are encoded as pulse detuning parameters within a Rydberg Hamiltonian, and quantum embeddings are subsequently obtained through expectation values. These embeddings are then passed to a linear classifier. Our simulations show that this method outperforms some traditional approaches that use PCA or unguided autoencoders. We also conduct ablation studies to assess the impact of various quantum and training parameters, demonstrating the robustness and flexibility of our proposed pipeline for real-world medical imaging applications, even in the current NISQ era.

==> images/diagrams/autoencoder_architecture.tex <==
% FIND WHITE NODES

\begin{figure}[!tb]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{circuitikz}
            \tikzstyle{every node}=[font=\LARGE]
            \draw[ fill={rgb,255:red,246; green,245; blue,244} ] (4.25,11.75) rectangle (5.5,10.5);
            \draw[ fill={rgb,255:red,246; green,245; blue,244} ] (4.75,11.25) rectangle (6,10);
            \node[font=\LARGE] at (5,12.25) {$\mathbf{x}$};
            \draw[->, >=Stealth] (6,11) -- (8,11);
            \draw(8,12.25) rectangle  node {\Huge $f_{\bm\theta}(\bm{x})$} (10.5,9.75);
            \node[font=\large] at (9.5,11.25) {};
            \node[font=\large] at (9,10.5) {};
            \node[font=\large] at (10.5,11.25) {};
            \draw[short] (13.75,11.5) -- (10.5,12.25);
            \draw[short] (10.5,9.75) -- (13.75,10.5);
            \draw(13.75,11.75) rectangle  node {\LARGE $\bm{z}$} (14.5,10);
            \draw(17.75,12.25) rectangle  node {\Huge $g_{\bm\phi}(\bm{z})$} (20.25,9.75);
            \draw[short] (17.75,12.25) -- (14.5,11.5);
            \draw[short] (14.5,10.5) -- (17.75,9.75);
            \node[font=\Large] at (14,13.75) {Autoencoder};
            \node[font=\large] at (10,12.75) {Encoder Network};
            \node[font=\large] at (18.25,12.75) {Decoder Network};
            \draw[->, >=Stealth] (20.25,11) -- (22.25,11);
            \draw[ fill={rgb,255:red,154; green,153; blue,150} ] (22.75,11.75) rectangle (24,10.5);
            \draw[ fill={rgb,255:red,154; green,153; blue,150} ] (22.25,11.25) rectangle (23.5,10);
            \node[font=\LARGE] at (23,12.25) {$\bm{\hat{x}}$};
            \draw[<->, >=Stealth, dashed] (5.25,11.75) .. controls (7.5,16.25) and (21.75,15.75) .. (23,11.75)node[pos=0.5, fill=white]{$\mathcal{L}$};
            %\node[font=\huge] at (17.75,51.5) {};
            \node[font=\Large] at (14,12.25) {Latent};
        \end{circuitikz}
    }%
    
\caption{
    Autoencoder architecture. The encoder network $f_{\bm\theta}(\bm{x})$ 
    compresses the input $\bm{x}$ into a latent representation $\bm{z}$, while the decoder 
    network $g_{\bm\phi}(\bm{z})$ reconstructs the input from the latent representation, 
    producing $\hat{x}$. The reconstruction loss $\mathcal{L}$ measures the 
    compresses the input $\bm{x}$ into a latent representation $\bm{z}$, while the decoder 
    network $g_{\bm\phi}(\bm{z})$ reconstructs the input from the latent representation, 
    producing $\hat{\bm{x}}$.
}
\label{fig:autoencoder_architecture}
\end{figure}
